Social Media Monitoring for IoT Cyber-Threats

The rapid development of IoT applications and their use in various fields of everyday life has resulted in an escalated number of different possible cyber-threats, and has consequently raised the need of securing IoT devices. Collecting Cyber-Threat Intelligence (e.g., zero-day vulnerabilities or trending exploits) from various online sources and utilizing it to proactively secure IoT systems or prepare mitigation scenarios has proven to be a promising direction. In this work, we focus on social media monitoring and investigate real-time Cyber-Threat Intelligence detection from the Twitter stream. Initially, we compare and extensively evaluate six different machine-learning based classification alternatives trained with vulnerability descriptions and tested with real-world data from the Twitter stream to identify the best-fitting solution. Subsequently, based on our findings, we propose a novel social media monitoring system tailored to the IoT domain; the system allows users to identify recent/trending vulnerabilities and exploits on IoT devices. Finally, to aid research on the field and support the reproducibility of our results we publicly release all annotated datasets created during this process.

==> sec6/sec6.tex <==
\section{Summary of results} \label{sec:summary}

\begin{enumerate}
\item We used data with \textit{different formats} as training and testing datasets; we managed to verify a model that performs well even with the unformatted Twitter data.

\item We constructed and published on GitHub \textit{two annotated datasets} that contain tweets related and unrelated to IoT vulnerabilties.

\item Contrary to previous studies, we used \textit{balanced datasets}, in terms of related and unrelated entries, in the training process.

\item As far as we know, this is the \textit{first approach that detects IoT vulnerabilities on Twitte}r, also being \textit{trained with CVE records} and \textit{tested with actual Twitter data}, whereas current state-of-the-art studies (i) either detect non-IoT-specific vulnerabilities from Twitter stream, (ii) classify software or other vulnerabilites by using as testing datasets bugs reports, CVE records, etc., or (iii) categorise IoT vulnerabilites by using CVE records as the testing dataset.

\item The evaluation process \textit{highlighted the Random Forest classifier}, contrary to previous studies, which ouperformed all its competitors for all versions of training data and for all performance measures. % other classification models like SVM (in most cases), Naive bayes, CNN, etc had the best performance whereas in our case Random Forest had the best score.\\

\item We propose a \textit{social media monitoring system} that uses the no CVE-tagged trained Random Forest model and focuses on real-time event detection from Twitter streams using state-of-the-art tools from the data science domain to automatically classify posts as related or unrelated to IoT vulnerabilities.
\end{enumerate}
